A Comparison of Common Users across Instagram and Ask.fm to Better Understand Cyberbullying

This paper examines users who are common to two popular online social networks, Instagram and Ask.fm, that are often used for cyberbullying. An analysis of the negativity and positivity of word usage in posts by common users of these two social networks is performed. These results are normalized in comparison to a sample of typical users in both networks. We also examine the posting activity of common user profiles and consider its correlation with negativity. Within the Ask.fm social network, which allows anonymous posts, the relationship between anonymity and negativity is further explored.

==> ack.tex <==
\section{Acknowledgements}

We wish to thank the National Science Foundation (NSF) for supporting this research with grant $\#$ (anonymized).




==> comparisonPositivity.tex <==
\section{Comparison of Positivity between Normal and Common Users}
To observe any potential influences of commonalities of a user across two social networks (Ask.fm and Instagram), we  studied the profile contents of the $10,000$
Common Users. Upon completion of collecting the profile contents of these users, we separated the posts present into two groups, posts by profile owners and posts by friends to
compare their individual positivity and negativity across Ask.fm and Instagram. Figure \ref{comm_neg} and \ref{comm_pos} shows the CCDF of the percentage of negative and positive posts by those Common Users and their friends in Ask.fm and Instagram respectively. Figure \ref{comm_neg} and \ref{comm_pos}  show that both for the case of posts by profile owners and posts or questions by friends, the negativity and positivity almost always follows the same pattern to each other. This finding clearly demonstrates that the commonality of users across Ask.fm and Instagram does not distinctly influence the negativity and positivity of their profile or in other words, common users tend to get the same positive and negative treatment across Ask.fm and Instagram.


==> datacollection.tex <==
\section{Data Collection}

   It could start by explaining the collection of normal users for each network, and then transition into the definition and motivation for common users, .
 
For the purpose of comparison of user behavior in a non-anonymous and semi anonymous social network, we are going to compare a set of user statistics in Instagram and ask.fm social networks. For Instagram users, starting from a seed node,41K user ids were gathered with snowball sampling method. Among these Instagram ids, there were both public and private profiles. We dont have access to shared media objects, comments and likes for private profiles. There the data would be limited to those users who have public profiles. For 41K users, only 61\% of them have public profiles which allows us access to their shared media objects, comments and likes. Therefore at the end around 25K complete user profile were collected for named as ``normal public Instagram" groups. For each public Instagram user, the collected data includes uesr id of follows, user id of followed by, comments and likes for all shared media objects. On the other hand, starting from a seed node, 17K complete Ask.fm profile were collected named as ``normal Ask.fm'' users group using the same approach as above. For each Ask.fm user, the profile information, complete list of questions, their answers and authors (if non-anonymized) and user id of people who have liked each answered+question is collected. 

After collectiong Ask.fm user Information we observed some users have revealed their instagram ids in their profile information. Selecting these users which we have both their Ask.fm and Instagram ids enables us to better compare two networks than comparing aggregates/averages of normal but non-common users. For this purpose tt the first step, starting from a seed node, we collected 1M users information using snowball sampling method. Only 4\% of the users have mentioned their Instagram id in their profile information which provide for us round 40K users with ids for two social networks. From these Instagram users we could obtain around 24K public profiles. These users with public profiles in both ask.fm and Instagram social network would be named as ``common public Instagram" and "common Ask.fm" users. Complete profile content for 8K users were collected for common users from each of the mentioned social network.
\comment{ we collect around 18K profile for Instagram and 10K (b/c of time limitation) from ask.fm which among those we have 8K common users}

For the rest of the paper, we will have our analysis in these four user groups.

We consider profanity words usage as a potential indicator of cyberbullying. Therefore we are mostly interested in the negative and positive words usage and the difference across Ask.fm and Instagram among common users. For this purpose we are using a dictionary of 1500 negative words (obtained from \cite{NegativeWordsList}) and 1500 positive words. Then we calculate the percentage of posts by profile owners and friends that include at least one of the words in our dictionaries and consider is as a measure of \textit{negativity} and \textit{positivity} of a profile.









==> howuserswereselected.tex <==
\section{How users were selected}
First we collected 17000 typical Ask.fm users' profile data. the users have been selected by snowballing the network. We also collected 10000 Ask.fm users who have also shared their Instagram profile information on their profile. We then collected the instagram and Ask.fm profile data of these users who will be referred in this paper as Common Instagram Users   and Common Ask.fm Users. We then collected over 20000 public typical Instagram users' profile data with the same way as the typical Ask.fm users. They will be referred in this paper as Typical Ask.fm Users and Typical Instagram Users. The reason for collecting data like this is twofold, to observe if the commonality of users in two social networks influence the negativity in their profiles and to observe the impact of anonymity on the negativity in their profile data by analyzing the common users in Ask.fm and Instagram which are semi-anonymous and non-anonymous networks respectively.



==> whythese.tex <==
\section{Study of Instagram and Ask.fm}

In order to analyze the influence of anonymity on the negativity of social networks, we chose Ask.fm and Instagram, a semi-anonymous and non-anonymous network respectively. Ask.fm is a social networking site where the users can ask other users questions with the option of anonymity. The profile owners' web pages only show the questions that have been answered and other users have the option of liking a particular post. Users also have the option to follow another user and send private, public or anonymous gifts to another user.

On the other hand, Instagram is an online mobile phot sharing, video sharing and social networking service that allows users to take pictures, apply digital filters to them and share them on other social networking sites such as Facebook, Flickr, Twitter and so on. Users can follow other users after their follow requests have been accepted, after which they can see the  media posts of that user. Upon opening a account, the default access privilege is public but users can change that to private which means only the people who are following them can see their posts. Users can like and comment on a media post and they can also tag other users while commenting. The fact that the name and the profile of the users who are liking and following and commenting is there for everyone to see, Instagram perfectly suits our criteria of being non-anonymous.

==> whythesenetworks.tex <==
% !TEX root = main.tex
\section{Instagram and Ask.fm Features}

%Compare here Instagram data and Ask.fm data.

We chose to study the user behavior in Instagram and Ask.fm because both of these networks are very popular among teenagers and have increasingly been used for cyberbullying. Furthermore, all user postings in these networks are publically
available.
%To better understand these networks as well as the results of our analysis below, we outline here some of the key characteristics of each network.
%In order to analyze the influence of anonymity on the negativity of social networks, we chose Ask.fm and Instagram, a semi-anonymous and non-anonymous network respectively. 
In Ask.fm, each user maintains his or her profile and other users can ask
questions by posting a question on that profile. By default, the identity of
the user asking questions is not revealed. Thus, Ask.fm is a semi-anonymous
network in which the identity of the profile owners is known but by default
the identity of the users asking questions is not known. Users asking questions have the option to reveal their identity however. {\bf In the Ask.fm data that
we analyzed, we noticed that about 10\% of the users chose to reveal their
identity. (We need to calculate it)} Profile owners may answer
some of the questions posted on their profile. Their web pages show only the
questions they choose to answer along with their answer. Users have the
option of liking a particular conversation consisting of a question and
answer pair which can not be done anonymously. They also
have the option to follow another user as well as send private, public or
anonymous gifts to the other users.

While Ask.fm is a web-based social network with textual content, Instagram
is a mobile social network that allows users to take pictures using their
smartphones, apply digital filters to them, post them as media on their
accounts, and share them on other social networking sites such as Facebook,
Flickr, Twitter and so on. Users can follow other users after their follow requests have been accepted. A user following another user can see the  media posts of that user. The default access privilege in Instagram is public, which means 
everyone can see the media objects posted by a user. However, users have
the option to change the access privilege to private, so that only the
people who are following them can see their posts. In the Instagram data
that we analyzed, we noticed that 49\% of users chose to keep their
access previlige private. Users in Instagram can like a media post, comment
on a media post, and can also tag other users while commenting. Unlike 
Ask.fm, Instagram is a completely non-anonymous network since the name and
the profile of the users who like, follow or comment are visible to everyone.

